Boosting Big Brother: Attacking Search Engines with Encodings

Search engines are vulnerable to attacks against indexing and searching via text encoding manipulation. By imperceptibly perturbing text using uncommon encoded representations, adversaries can control results across search engines for specific search queries. We demonstrate that this attack is successful against two major commercial search engines - Google and Bing - and one open source search engine - Elasticsearch. We further demonstrate that this attack is successful against LLM chat search including Bing's GPT-4 chatbot and Google's Bard chatbot. We also present a variant of the attack targeting text summarization and plagiarism detection models, two ML tasks closely tied to search. We provide a set of defenses against these techniques and warn that adversaries can leverage these attacks to launch disinformation campaigns against unsuspecting users, motivating the need for search engine maintainers to patch deployed systems.

==> figures/grammerly.tex <==
\begin{figure}[b]
    \centering
    \includegraphics[width = 0.95\linewidth]{figures/graphics/grammarly.pdf}
    \caption{Attack success rate (ASR) of imperceptible perturbations on Grammarly plagiarism checker.}
    \label{fig:grammarly-asr}
\end{figure}
